Sequential Nature of Recommender Systems Disrupts the Evaluation Process

Datasets are often generated in a sequential manner, where the previous samples and intermediate decisions or interventions affect subsequent samples. This is especially prominent in cases where there are significant human-AI interactions, such as in recommender systems. To characterize the importance of this relationship across samples, we propose to use adversarial attacks on popular evaluation processes. We present sequence-aware boosting attacks and provide a lower bound on the amount of extra information that can be exploited from a confidential test set solely based on the order of the observed data. We use real and synthetic data to test our methods and show that the evaluation process on the MovieLense-100k dataset can be affected by $\sim1\%$ which is important when considering the close competition. Codes are publicly available.

==> sections/old_abstract.tex <==
\begin{abstract}
The sequential information that lies in datasets collected through the interaction of humans and algorithms might disrupt the evaluation process. To characterize the importance of this information under different evaluation mechanisms, we suggest using adversarial attacks on the test set. Focusing on recommender systems, we propose sequence-aware boosting attacks to show a lower bound on the amount of extra information that can be exploited from a confidential test set solely based on the order of the observed data. We use real and synthetic data to test our methods and show that the evaluation process on the MovieLense-100k dataset can be affected by $\sim0.5\%$, which is important when considering the close competition. Codes are publicly available.\footnote{Due to anonymity policy, link to the codes is removed.}.

 
\keywords{Sequential Decision Making  \and Evaluation Mechanisms \and Missing-Not-At-Random}
\end{abstract}
